Learning Explainable and Better Performing Representations of POMDP Strategies

Strategies for partially observable Markov decision processes (POMDP) typically require memory. One way to represent this memory is via automata. We present a method to learn an automaton representation of a strategy using a modification of the L*-algorithm. Compared to the tabular representation of a strategy, the resulting automaton is dramatically smaller and thus also more explainable. Moreover, in the learning process, our heuristics may even improve the strategy's performance. In contrast to approaches that synthesize an automaton directly from the POMDP thereby solving it, our approach is incomparably more scalable.

==> format/spacing.tex <==
% SPACE HACKS
%\titlespacing*{\section}{0pt}{12pt plus 4pt minus 4pt}{12pt plus 2pt minus 2pt}
%\titlespacing*{\subsection}{0pt}{10pt plus 3pt minus 3pt}{10pt plus 2pt minus 1pt}
%\titlespacing\subsubsection{0pt}{8pt plus 2pt minus 2pt}{8pt plus 1pt minus 1pt}

%\renewcommand{\baselinestretch}{0.98} % >=0.97
\advance\textwidth3mm % <= 5mm
\advance\hoffset-1.5mm
\advance\textheight1mm
%\advance\voffset-3mm

%\setlength{\marginparwidth}{3.3cm}
%\setlength{\marginparsep}{0.1cm}
%\setlength{\textfloatsep}{0.8\textfloatsep} % Space below/above a float if its [t]
%\setlength{\intextsep}{0.8\intextsep} % Space below/above a float if its [h]

\makeatletter
\renewcommand\section{\@startsection {section}{1}{\z@}%
      {-2ex \@plus -1ex \@minus -.2ex}% <beforeskip>
      {1ex \@plus .2ex}% <afterskip>
      {\normalfont\Large\bfseries\SS@sectfont}}
\renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
      {-2ex\@plus -1ex \@minus -.2ex}% <beforeskip>
      {1ex \@plus .2ex}% <afterskip>
      {\normalfont\large\bfseries\SS@subsectfont}}
\makeatother

% Gaps between titles

% \titlespacing*{<command>}{<left>}{<before-sep>}{<after-sep>}
%\titlespacing*{\section} {0pt}{3.5ex plus 1ex minus .2ex}{2.3ex plus .2ex}
% \titlespacing*{\subsection} {0pt}{3.25ex plus 1ex minus .2ex}{1.5ex plus .2ex}
% \titlespacing*{\subsubsection}{0pt}{3.25ex plus 1ex minus .2ex}{1.5ex plus .2ex}
% \titlespacing*{\paragraph} {0pt}{3.25ex plus 1ex minus .2ex}{1em}
% \titlespacing*{\subparagraph} {\parindent}{3.25ex plus 1ex minus .2ex}{1em}

% Alter some LaTeX defaults for better treatment of figures:
% See p.105 of "TeX Unbound" for suggested values.
% See pp. 199-200 of Lamport's "LaTeX" book for details.
%   General parameters, for ALL pages:
\renewcommand{\topfraction}{0.95}	% max fraction of floats at top
\renewcommand{\bottomfraction}{0.95}	% max fraction of floats at bottom
%   Parameters for TEXT pages (not float pages):
% \setcounter{topnumber}{2} % number of floats that can be displayed at the top
% \setcounter{bottomnumber}{2} % number of floats that can be displayed at the bottom
% \setcounter{totalnumber}{4}     % 2 may work better
% \setcounter{dbltopnumber}{2}    % for 2-column pages
% \renewcommand{\dbltopfraction}{0.9}	% fit big float above 2-col. text
\renewcommand{\textfraction}{0.07}	% allow minimal text w. figs
%   Parameters for FLOAT pages (not text pages):
\renewcommand{\floatpagefraction}{0.95}	% require fuller float pages
% N.B.: floatpagefraction MUST be less than topfraction !!
% \renewcommand{\dblfloatpagefraction}{0.7}	% require fuller float pages
% remember to use [htp] or [htpb] for placement


% A good document on space hacks
% http://www-h.eng.cam.ac.uk/help/tpl/textprocessing/squeeze.html


% space left between floats (12.0pt plus 2.0pt minus 2.0pt).
\setlength{\floatsep}{10pt}
% space between last top float or first bottom float and the text (20.0pt plus 2.0pt minus 4.0pt).
\setlength{\textfloatsep}{16pt}
% space left on top and bottom of an in-text float (12.0pt plus 2.0pt minus 2.0pt).
\setlength{\intextsep}{10pt}
%\dbltextfloatsep is \textfloatsep for 2 column output (20.0pt plus 2.0pt minus 4.0pt).
%\dblfloatsep is \floatsep for 2 column output (12.0pt plus 2.0pt minus 2.0pt).
% space above caption (10.0pt).
\setlength{\abovecaptionskip}{10pt}
% space below caption (0.0pt).
\setlength{\belowcaptionskip}{0pt}
